Actionable Conversational Quality Indicators for Improving Task-Oriented Dialog Systems

Automatic dialog systems have become a mainstream part of online customer service. Many such systems are built, maintained, and improved by customer service specialists, rather than dialog systems engineers and computer programmers. As conversations between people and machines become commonplace, it is critical to understand what is working, what is not, and what actions can be taken to reduce the frequency of inappropriate system responses. These analyses and recommendations need to be presented in terms that directly reflect the user experience rather than the internal dialog processing. This paper introduces and explains the use of Actionable Conversational Quality Indicators (ACQIs), which are used both to recognize parts of dialogs that can be improved, and to recommend how to improve them. This combines benefits of previous approaches, some of which have focused on producing dialog quality scoring while others have sought to categorize the types of errors the dialog system is making. We demonstrate the effectiveness of using ACQIs on LivePerson internal dialog systems used in commercial customer service applications, and on the publicly available CMU LEGOv2 conversational dataset (Raux et al. 2005). We report on the annotation and analysis of conversational datasets showing which ACQIs are important to fix in various situations. The annotated datasets are then used to build a predictive model which uses a turn-based vector embedding of the message texts and achieves an 79% weighted average f1-measure at the task of finding the correct ACQI for a given conversation. We predict that if such a model worked perfectly, the range of potential improvement actions a bot-builder must consider at each turn could be reduced by an average of 81%.

==> model_perf_no_pearson.tex <==

\begin{table*}[!ht]
\caption{IQ Model Performance: linear weighted Cohen kappa (LWCK), unweighted average recall (UAR), Spearman rank correlation ($\rho$) for IQ. Model Selection and Hyper-parameter selection was accomplished by nested cross-validation (5 folds).}
\label{tab:iq_model_performance}

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
  \textbf{Dialog System} &        \textbf{Features Used} & \textbf{Spearman} &   \textbf{UAR} & \textbf{Pearson} &  \textbf{LWCK} \\ \hline

\multirow{ 5}{*}{CMU} & text &    0.572 & 0.585 &   0.532 &  0.47 \\ \cline{2-6}
 & only-gold-cqi &    0.469 & 0.499 &   0.477 & 0.404 \\ \cline{2-6}
 & only-pred-cqi &    0.296 & 0.396 &   0.222 & 0.242 \\ \cline{2-6}
 & gold-cqi+text &    0.622 & 0.597 &    0.56 & 0.529 \\ \cline{2-6}
 & pred-cqi+text &    0.593 & 0.516 &   0.517 & 0.475 \\ \hline

\multirow{ 5}{*}{Junior Sales Assistant} & text &    0.721 & 0.567 &   0.605 & 0.678 \\ \cline{2-6}
 & only-gold-cqi &    0.147 & 0.429 &   0.163 & 0.349 \\ \cline{2-6}
 & only-pred-cqi &    0.529 & 0.399 &    0.47 & 0.494 \\ \cline{2-6}
 & gold-cqi+text &     0.84 & 0.599 &    0.77 & 0.797 \\ \cline{2-6}
 & pred-cqi+text &    0.831 & 0.573 &   0.789 & 0.798 \\ \hline

\multirow{ 5}{*}{Help and Route} &  text &    0.569 & 0.503 &   0.528 & 0.495 \\ \cline{2-6}
& only-gold-cqi &     0.25 & 0.363 &   0.288 & 0.285 \\ \cline{2-6}
& only-pred-cqi &    0.288 & 0.384 &    0.22 & 0.256 \\ \cline{2-6}
 & gold-cqi+text &    0.673 & 0.553 &   0.643 & 0.597 \\  \cline{2-6}
  & pred-cqi+text &    0.682 & 0.434 &    0.64 & 0.583 \\ \hline


 \multirow{ 5}{*}{Router} & text &    0.621 & 0.346 &   0.558 & 0.585 \\ \cline{2-6}
 & only-gold-cqi &    0.608 & 0.482 &   0.604 & 0.521 \\ \cline{2-6}
 & only-pred-cqi &    0.636 & 0.341 &   0.516 & 0.592 \\ \cline{2-6}
 & gold-cqi+text &    0.765 & 0.635 &   0.701 & 0.679 \\ \cline{2-6}
 & pred-cqi+text &    0.841 & 0.374 &   0.723 & 0.791 \\ \hline

 \multirow{ 5}{*}{Food Expert} &  text &    0.698 & 0.603 &    0.65 & 0.609 \\ \cline{2-6}
 & only-gold-cqi &    0.574 & 0.469 &   0.481 & 0.493 \\ \cline{2-6}
 & only-pred-cqi &    0.514 & 0.435 &   0.428 & 0.448 \\ \cline{2-6}
 & gold-cqi+text &    0.765 & 0.635 &   0.701 & 0.679 \\ \cline{2-6}
 & pred-cqi+text &    0.787 &  0.55 &   0.682 & 0.691 \\ \hline
\hline
 \multirow{ 5}{*}{All Bots} & text &    0.595 & 0.599 &    0.55 & 0.499 \\ \cline{2-6}
  & only-gold-cqi &    0.462 & 0.511 &    0.48 & 0.417 \\ \cline{2-6}
  & only-pred-cqi &    0.326 & 0.408 &   0.241 & 0.274 \\ \cline{2-6}
  &      gold-cqi+text &    0.651 & 0.612 &   0.583 & 0.561 \\ \cline{2-6}
  &      pred-cqi+text &    0.624 & 0.531 &   0.537 & 0.514 \\ \hline
% \bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}



new old
combined

\begin{table*}[!ht]
\caption{IQ Model Performance: linear weighted Cohen kappa (LWCK), unweighted average recall (UAR), Spearman rank correlation ($\rho$) for IQ. Model Selection and Hyper-parameter selection was accomplished by nested cross-validation (5 folds).}
\label{tab:iq_model_performance}

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|l|l|l|l|}
\hline
  \textbf{Dialog System} &        \textbf{Features Used} & \textbf{$\rho$} &   \textbf{UAR} &  \textbf{LWCK} \\ \hline

\multirow{ 5}{*}{CMU} & text &    0.572 & 0.585  &  0.47 \\ \cline{2-5}
 & only-gold-cqi &    0.469 & 0.499 &    0.404 \\ \cline{2-5}
 & only-pred-cqi &    0.296 & 0.396 &    0.242 \\ \cline{2-5}
 & gold-cqi+text &    0.622 & 0.597 &    0.529 \\ \cline{2-5}
 & pred-cqi+text &    0.593 & 0.516 &    0.475 \\ \hline

\multirow{ 5}{*}{Junior Sales Assistant} & text &    0.721 & 0.567 &  0.678 \\ \cline{2-5}
 & only-gold-cqi &    0.147 & 0.429 &    0.349 \\ \cline{2-5}
 & only-pred-cqi &    0.529 & 0.399 &     0.494 \\ \cline{2-5}
 & gold-cqi+text &     0.84 & 0.599 &     0.797 \\ \cline{2-5}
 & pred-cqi+text &    0.831 & 0.573 &    0.798 \\ \hline

\multirow{ 5}{*}{Help and Route} &  text &    0.569 & 0.503 &    0.495 \\ \cline{2-5}
& only-gold-cqi &     0.25 & 0.363 &    0.285 \\ \cline{2-5}
& only-pred-cqi &    0.288 & 0.384 &    0.256 \\ \cline{2-5}
 & gold-cqi+text &    0.673 & 0.553 &   0.597 \\  \cline{2-5}
  & pred-cqi+text &    0.682 & 0.434 &    0.583 \\ \hline


 \multirow{ 5}{*}{Router} & text &    0.621 & 0.346 &  0.585 \\ \cline{2-5}
 & only-gold-cqi &    0.608 & 0.482 &   0.521 \\ \cline{2-5}
 & only-pred-cqi &    0.636 & 0.341 &   0.592 \\ \cline{2-5}
 & gold-cqi+text &    0.765 & 0.635 &   0.679 \\ \cline{2-5}
 & pred-cqi+text &    0.841 & 0.374 &   0.791 \\ \hline

 \multirow{ 5}{*}{Food Expert} &  text &    0.698 & 0.603 &   0.609 \\ \cline{2-5}
 & only-gold-cqi &    0.574 & 0.469 & 0.493 \\ \cline{2-5}
 & only-pred-cqi &    0.514 & 0.435 &  0.448 \\ \cline{2-5}
 & gold-cqi+text &    0.765 & 0.635 &  0.679 \\ \cline{2-5}
 & pred-cqi+text &    0.787 &  0.55 &  0.691 \\ \hline
\hline
 \multirow{ 5}{*}{All Bots} & text &    0.595 & 0.599 &  0.499 \\ \cline{2-5}
  & only-gold-cqi &    0.462 & 0.511 &  0.417 \\ \cline{2-5}
  & only-pred-cqi &    0.326 & 0.408 &  0.274 \\ \cline{2-5}
  &      gold-cqi+text &    0.651 & 0.612 &  0.561 \\ \cline{2-5}
  &      pred-cqi+text &    0.624 & 0.531 &  0.514 \\ \hline
% \bottomrule
\end{tabular}
\quad
\begin{tabular}{|l|r|r|r|r|}
\hline
                      \textbf{ACQI} &  \textbf{Precision} &  \textbf{Recall} &  \textbf{F1-score} &  \textbf{Support} \\ \hline
       Ask for Information &      0.948 &   0.896 &     0.921 &   4144 \\ \hline
      Ask for Confirmation &      0.777 &   0.781 &     0.779 &   2069 \\ \hline
       Does Not Understand &      0.524 &   0.495 &     0.509 &   1417 \\ \hline
       Provides Assistance &      0.884 &   0.902 &     0.893 &   1010 \\ \hline
Ignored Consumer Statement &      0.196 &   0.270 &     0.227 &    226 \\ \hline
         Unable to Resolve &      0.599 &   0.807 &     0.688 &    176 \\ \hline
            Input Rejected &      0.236 &   0.392 &     0.295 &    120 \\ \hline
                   Restart &      0.484 &   0.762 &     0.592 &     80 \\ \hline
              Bad Transfer &      0.250 &   0.286 &     0.267 &     14 \\ \hline \hline
   macro avg &      0.544 &   0.621 &     0.574 & 9256 \\ \hline
weighted avg &      0.799 &   0.784 &     0.790 & 9256 \\ \hline

\end{tabular}

\end{center}
\end{footnotesize}
\end{table*}


%
\subsection{Predicting ACQI: Results and Discussion}

For the IQ prediction experiment, results for each of the \bots using only text-derived features and 
logistic regression as a classifier (as described above) are presented in Table \ref{tab:iq_model_performance}.

Points to note include:

\begin{itemize}
    \item The overall weighted average f1-score is 0.790. We are predicting the correct ACQI nearly 80\% of the time overall.
    \item The accuracy of the classification depends significantly on the support of the class: common ACQIs are predicted much more accurately 
    that rare ones.
    \item Because of this, the macro average performance (not weighted by support) is worse, with an f1-score of just 0.574.
    \item The score can be cross-referenced against Figure \ref{fig:score_change_dist} and Table \ref{tab:dist_ACQI_given_score_decrease} to guide improvement efforts. For example, `Does Not Understand' occurs relatively frequently and with overwhelmingly negative impact on IQ score, but the F1-score for predicting this
    class is only 0.509. Improving ACQI classification performance for this class would therefore be especially impactful.
\end{itemize}

\begin{table*}[!ht]
\begin{center}
\caption{ACQI Model Performance}
\label{tab:cqi_model_performance}
\begin{footnotesize}
\begin{tabular}{|l|r|r|r|r|}
\hline
                      \textbf{ACQI} &  \textbf{Precision} &  \textbf{Recall} &  \textbf{F1-score} &  \textbf{Support} \\ \hline
       Ask for Information &      0.948 &   0.896 &     0.921 &   4144 \\ \hline
      Ask for Confirmation &      0.777 &   0.781 &     0.779 &   2069 \\ \hline
       Does Not Understand &      0.524 &   0.495 &     0.509 &   1417 \\ \hline
       Provides Assistance &      0.884 &   0.902 &     0.893 &   1010 \\ \hline
Ignored Consumer Statement &      0.196 &   0.270 &     0.227 &    226 \\ \hline
         Unable to Resolve &      0.599 &   0.807 &     0.688 &    176 \\ \hline
            Input Rejected &      0.236 &   0.392 &     0.295 &    120 \\ \hline
                   Restart &      0.484 &   0.762 &     0.592 &     80 \\ \hline
              Bad Transfer &      0.250 &   0.286 &     0.267 &     14 \\ \hline \hline
   macro avg &      0.544 &   0.621 &     0.574 & 9256 \\ \hline
weighted avg &      0.799 &   0.784 &     0.790 & 9256 \\ \hline

\end{tabular}
\end{footnotesize}
\end{center}
\end{table*}
